Think, Prune, Train, Improve: Scaling Reasoning without Scaling Models

Large language models (LLMs) have demonstrated strong capabilities in programming and mathematical reasoning tasks, but are constrained by limited high-quality training data. Synthetic data can be leveraged to enhance fine-tuning outcomes, but several factors influence this process, including model size, synthetic data volume, pruning strategy, and number of fine-tuning rounds. We explore these axes and investigate which conditions enable model self-improvement. We introduce the Think, Prune, Train process, a scalable framework that iteratively fine-tunes models on their own reasoning traces, using ground-truth pruning to ensure high-quality training data. This approach yields improved performance: on GSM8K, Gemma2-2B achieves a Pass@1 of 57.6% (from 41.9%), Gemma2-9B reaches 82%, matching LLaMA-3.1-70B, and LLaMA-3.1-70B attains 91%, even surpassing GPT-4o, demonstrating the effectiveness of self-generated reasoning and systematic data selection for improving LLM capabilities.

==> assets/comparison_human_self_distill.tex <==

\label{scalingsynth}
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.5 \textwidth,
            height=0.3\textwidth,
            xlabel={Number of Training Examples},
            ylabel={GSM8K Pass@1(\%)},
            ymin=40, ymax=60,
            xmin=1.5, xmax=6.5,
            xtick={2,4,6},
            xticklabels={2k, 4k, 6k},
            grid=major,
            legend style={at={(0.5,-0.25)}, anchor=north, legend columns=-1}
        ]
            % 2B Synthetic
            \addplot[
                blue,
                mark=*,
                thick
            ] coordinates {
                (2, 52.5)
                (4, 54.8)
                (6, 51.6)
            };
            \addlegendentry{2b-generated data}
            
            % 9B Synthetic
            \addplot[
                green,
                mark=triangle*,
                thick
            ] coordinates {
                (2, 54.0)
                (4, 53.1)
                (6, 51.2)
            };
            \addlegendentry{9b-generated data}
            
            % Baseline reference
            \draw[dashed] (axis cs:1.5,41.9) -- (axis cs:6.5,41.9)
                node[pos=0.85, anchor=south, font=\tiny] {Gemma 2-2b Baseline (41.9\%)};
        \end{axis}
    \end{tikzpicture}
    \caption{\textbf{Scaling synthetic training dataset size across model Sizes show similar performance, but no clear trends, motivating a different solution.} 
    Pass@1(\%) performance comparison of fine-tuned 2B models on GSM8K using self-generated data from the 2B model and distilled data from the 9B model.}
    \label{fig:pass1_gsm8k}
\end{figure}


==> assets/prompt.tex <==


\begin{tcolorbox}[colback=blue!5!white, colframe=blue!75!black, title=\tiny{Mathematical Reasoning Prompt}, scale=0.2]
\tiny
\textbf{You are an expert mathematician.}  

You are provided with a math problem.  
Your task is to solve the problem step-by-step, clearly showing all relevant calculations and reasoning.  

\vspace{0.1cm}
\noindent\textbf{Problem:}  
\texttt{"Bella bought stamps at the post office. Some of the stamps had a snowflake design, some had a truck design, and some had a rose design. Bella bought 11 snowflake stamps. She bought 9 more truck stamps than snowflake stamps, and 13 fewer rose stamps than truck stamps. How many stamps did Bella buy in all?"}

\vspace{0.1cm}
\noindent\textbf{Requirements:}
\begin{enumerate}
    \item Provide a complete and correct solution in a markdown block.
    \item Explain each step of the solution in detail.
    \item Conclude with the final numerical answer on a new line in the format \texttt{\#\#\#\# [Answer]}, replacing \texttt{[Answer]} with the actual answer.
\end{enumerate}

\vspace{0.1cm}
\noindent\textbf{Solution:}  
\end{tcolorbox}

==> assets/traces.tex <==

\begin{minipage}{0.48\textwidth}
\begin{tcolorbox}[colback=blue!5!white, colframe=blue!75!black, title=Gemma 2B]
\tiny
\textbf{Solution:}
\texttt{Here's a step-by-step solution to the problem: \\
        **1. Calculate the number of truck stamps:**
        * Bella bought 9 more truck stamps than snowflake stamps, and she bought 11 snowflake stamps.
        * Therefore, she bought 11 + 9 = 20 truck stamps. \\
        **2. Calculate the number of rose stamps:*** Bella bought 13 fewer rose stamps than truck stamps, and she bought 20 truck stamps.\\* Therefore, she bought 20 - 13 = 7 rose stamps.\\
        **3. Calculate the total number of stamps:** \\
        * Bella bought 11 snowflake stamps + 20 truck stamps + 7 rose stamps = 38 stamps in total.\\ ** \#\#\#\# 38**}
\end{tcolorbox}

\begin{tcolorbox}[colback=green!5!white, colframe=green!75!black, title=Gemma 9B]
\tiny
\textbf{Solution:}
\tiny
\texttt{
Here's the step-by-step solution to the problem:\\
1.**Find the number of truck stamps:** \\
* Bella bought 9 more truck stamps than snowflake stamps, which she bought 11 of.\\
* Therefore, she bought 11 + 9 = 20 truck stamps.\\
2. **Find the number of rose stamps:**\\   * Bella bought 13 fewer rose stamps than truck stamps, which she bought 20 of.\\
* Therefore, she bought 20 - 13 = 7 rose stamps.\\
3. **Calculate the total number of stamps:** \\
* To find the total number of stamps, add the number of each type of stamp: 11 snowflake stamps + 20 truck stamps + 7 rose stamps = 38 stamps.\\ \#\#\#\# 38}
\end{tcolorbox}

\begin{tcolorbox}[colback=red!5!white, colframe=red!75!black, title=LLaMA 70B]
\tiny
\textbf{Solution:}
\texttt{\#\#\# Step-by-step solution to the problem\\ To find the total number of stamps Bella bought, we first need to determine the number of stamps for each design. We are given the following information:\\- The number of snowflake stamps = 11\\- The number of truck stamps = 9 more than snowflake stamps\\- The number of rose stamps = 13 fewer than truck stamps\\ \#\#\#  Calculating the number of truck stamps\\ Since Bella bought 9 more truck stamps than snowflake stamps, we calculate the number of truck stamps by adding 9 to the number of snowflake stamps.\\ Number of truck stamps = Number of snowflake stamps + 9\\= 11 + 9\\= 20\\ \#\#\#  Calculating the number of rose stamps\\ Given that Bella bought 13 fewer rose stamps than truck stamps, we calculate the number of rose stamps by subtracting 13 from the number of truck stamps.\\ Number of rose stamps = Number of truck stamps - 13\\ = 20 - 13\\ = 7\\\#\#\#  Calculating the total number of stamps\\ To find the total number of stamps, we add the number of snowflake, truck, and rose stamps together.\\ Total number of stamps = Number of snowflake stamps + Number of truck stamps + Number of rose stamps\\= 11 + 20 + 7\\= 38\\\#\#\#\# 38}
\end{tcolorbox}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\begin{tcolorbox}[colback=yellow!5!white, colframe=yellow!75!black, title=LLaMA 1B]
\tiny
\textbf{Solution:}
\texttt{\#\#\# Step 1: Interpret the Problem and Identify Given Information ...\#\#\# Step 2: Set Up Equations Based on Given Information\\From the problem, we can set up the following equations:\\1. `s = 11` (number of snowflake stamps)\\2. `t = s + 9` (number of truck stamps)\\3. `r = t - 13` (number of rose stamps)\\\\\#\#\# Step 3: Express the Number of Rose Stamps in Terms of Snowflake Stamps and Truck Stamps\\Now, we'll substitute the expressions for `t` and `r` into the third equation:\\\\`s = 11`\\`t = s + 9`\\`r = (s + 9) - 13`\\\\\#\#\# Step 4: Solve for the Number of Rose Stamps\\Let's simplify the expression for `r`:\\`r = (s + 9) - 13`\\`r = s - 4`\\\\So, the number of rose stamps in terms of the number of snowflake stamps is `r = s - 4`.\\\\\#\#\# Step 5: Find the Total Number of Stamps\\The total number of stamps is the sum of snowflake stamps, truck stamps, and rose stamps. Therefore, we can write an equation representing the total number of stamps:\\\\`s + t + r = 11 + (11 + 9) + (s - 4)`\\\\Simplify and solve for `s` (snowflake stamps):\\`s + t + r = 11 + 20 + s - 4`\\`s + t + r = 26 + s`\\`s - s = 26`\\`s = 26`
 \\\\Since `s` represents the number of snowflake stamps and we know `s = 11`, the actual number of snowflake stamps is indeed 11. Let's confirm this with the other equations.\\\\\#\#\# Step 6: Confirm the Number of Truck and Rose Stamps\\Now, we'll find the number of truck stamps `t` and rose stamps `r` using the equations:\\`t = s + 9`\\`r = t - 13`\\\\We found `s = 11`, so:\\`t = 11 + 9`\\`t = 20`\\\\`r = 20 - 13`\\`r = 7`\\\\ \#\# Step 7: Verify the Total Number of Stamps Calculations\\To ensure the correctness of our solution:\\`s + t + r = 11 + 20 + 7`\\`s + t + r = 38`\\\\Using the original formula `20 + 7 - 4 = 37`, this confirms our conclusion that `s = 11` is a perfect and easy-to-explain solution that satisfies all given conditions.\\\\\#\#\# Step 8: Conclusion with the Final Answer\\We finally have the total number of stamps Bella bought in all - 11 snowflake stamps, 20 truck stamps, and 7 rose stamps.\\\\\#\#\#\# 38
}
\end{tcolorbox}
\end{minipage}

%idk. 


\begin{figure}[h]
    \centering
    % Code Contest (CC) Graph
    % GSM8K Graph
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=1.1\textwidth,
                height=0.8\textwidth,
                xlabel={},
                ylabel={Pass@20\%},
                ymin=0, ymax=100,
                xtick={0, 1, 2, 3},
                xticklabels={
                    {2b GSM8K}, {2k np GSM8K}, {6k np GSM8K}, {Best ft 2b}
                },
                xticklabel style={rotate=45, anchor=east, font=\scriptsize},
                bar width=8pt,
                nodes near coords,
                every node near coord/.append style={font=\tiny},
                legend style={font=\tiny, at={(0.5,-0.4)}, anchor=north, legend columns=-1}
            ]

                % Baseline Data for GSM8K
                \addplot[
                    ybar,
                    color=blue,
                    fill=blue!30
                ] coordinates {
                    (0, 76.0) % Baseline GSM8K
                };
                \addlegendentry{Baseline GSM8K}

                % No Prune Data for GSM8K
                \addplot[
                    ybar,
                    color=red,
                    fill=red!30
                ] coordinates {
                    (1, 71.60) % 2k np GSM8K
                    (2, 71.00) % 6k np GSM8K
                };
                \addlegendentry{No Prune GSM8K}

                % Best Recur Data for GSM8K
                \addplot[
                    ybar,
                    color=green,
                    fill=green!30
                ] coordinates {
                    (3, 90.2) % Best Recur GSM8K
                };
                \addlegendentry{Best fine tuned 2b model GSM8K}

            \end{axis}
        \end{tikzpicture}
        \caption{Pass@20\% for GSM8K.}
        \label{fig:pass20_gsm8k}
    \end{subfigure}

    \caption{Comparison of performance metrics noprune GSM8K (Pass@20\%).}
    \label{fig:comparison_cc_gsm8k}
\end{figure}
